DIETA: A Decoder-only transformer-based model for Italian-English machine TrAnslation

In this paper, we present DIETA, a small, decoder-only Transformer model with 0.5 billion parameters, specifically designed and trained for Italian-English machine translation. We collect and curate a large parallel corpus consisting of approximately 207 million Italian-English sentence pairs across diverse domains, including parliamentary proceedings, legal texts, web-crawled content, subtitles, news, literature and 352 million back-translated data using pretrained models. Additionally, we create and release a new small-scale evaluation set, consisting of 450 sentences, based on 2025 WikiNews articles, enabling assessment of translation quality on contemporary text. Comprehensive evaluations show that DIETA achieves competitive performance on multiple Italian-English benchmarks, consistently ranking in the second quartile of a 32-system leaderboard and outperforming most other sub-3B models on four out of five test suites. The training script, trained models, curated corpus, and newly introduced evaluation set are made publicly available, facilitating further research and development in specialized Italian-English machine translation. https://github.com/pkasela/DIETA-Machine-Translation

==> tables/Datasets.tex <==
\begin{table}[ht]
\caption{Statistics of News dataset used for generating synthetic data.}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccc}
\toprule
\textbf{Language} & \textbf{News Year} & \textbf{N. of Sentences}  \\
\midrule
Italian & 2008 & 770653  \\  
Italian & 2009 & 3811046  \\
Italian & 2010 & 2302226  \\
Italian & 2011 & 5334067 \\
Italian & 2012 & 4379374 \\
Italian & 2013 & 4820207 \\
Italian & 2014 & 3447581 \\
Italian & 2015 & 2906264 \\
Italian & 2016 & 2168440 \\
Italian & 2017 & 2704992 \\
Italian & 2018 & 2760216 \\
Italian & 2019 & 4879057 \\
Italian & 2020 & 5825952 \\
Italian & 2021 & 4573401 \\
Italian & 2022 & 4630655 \\
Italian & 2023 & 6366126 \\
Italian & 2024 & 6159432 \\ \midrule
\textbf{Italian} & \textbf{Total} & 67839689  \\ \midrule
English & 2023 &  41263707 \\
English & 2024 & 35092299 \\ \midrule
\textbf{English} & \textbf{Total} &  76356006 \\ \bottomrule
\end{tabular}
\label{Table:datasets}
}
\end{table}

% \begin{table*}[ht]
% \caption{Statistics of datasets used for training our model: we report the name of the datasets, its domain, the number of sentence pairs after the filtering process and the percentage over the total number of pairs in de dataset.}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccccccc}
% \toprule
% \textbf{} & CCMatrix & Europarl & JRC-Acquis & OpenSubtitles & ParaCrawl & WikiMatrix & CCAligned & LinguaTools-WikiTitles \\
% \midrule
% Domain &  & Political & Political & Movie & Web & Wikipedia &  &  \\
% Sentence pairs (M) & 140 & 1.9 & 0.8 & 72 & 97 & 2.1 & 14 & 11.5 \\
% Percentage &  &  &  &  &  &  &  &  \\
% \midrule
% \textbf{} & EUbookshop & XLEnet & DGT & TildeMODEL & ELRC-EUIPO\_law & EMEA & Wikipedia & ELRC-2710-EMEA \\
% Domain &  &  &  &  &  &  &  &  \\
% Sentence pairs (M) & 6.5 & 6 & 5 & 3.7 & 1.2 & 1 & 0.96 & 0.8 \\
% Percentage &  &  &  &  &  &  &  &  \\
% \midrule
% \textbf{} & QED & wikimedia & TED2020 & GNOME & ELRC & KDE4 & NeuLab-TedTalks & ECB \\
% Domain &  &  &  &  &  &  &  &  \\
% Sentence pairs (M) & 0.6 & 0.6 & 0.3 & 0.3 &  & 0.2 & 0.2 & 0.2 \\
% Percentage &  &  &  &  &  &  &  &  \\
% \midrule
% \textbf{} & News-Commentary & ELITR-ECA & bible-uedin & PHP &  &  &  &  \\
% Domain &  &  &  &  &  &  &  &  \\
% Sentence pairs (M) & 0.08 &  & 0.06 & 0.03 &  &  &  &  \\
% Percentage &  &  &  &  &  &  &  &  \\
% \bottomrule
% \end{tabular}%
% }
% \label{Table:datasets}
% \end{table*}
